On Preserving the Behavior in Software Refactoring: A Systematic Mapping Study

Context: Refactoring is the art of modifying the design of a system without altering its behavior. The idea is to reorganize variables, classes and methods to facilitate their future adaptations and comprehension. As the concept of behavior preservation is fundamental for refactoring, several studies, using formal verification, language transformation and dynamic analysis, have been proposed to monitor the execution of refactoring operations and their impact on the program semantics. However, there is no existing study that examines the available behavior preservation strategies for each refactoring operation. Objective: This paper identifies behavior preservation approaches in the research literature. Method: We conduct, in this paper, a systematic mapping study, to capture all existing behavior preservation approaches that we classify based on several criteria including their methodology, applicability, and their degree of automation. Results: The results indicate that several behavior preservation approaches have been proposed in the literature. The approaches vary between using formalisms and techniques, developing automatic refactoring safety tools, and performing a manual analysis of the source code. Conclusion: Our taxonomy reveals that there exist some types of refactoring operations whose behavior preservation is under-researched. Our classification also indicates that several possible strategies can be combined to better detect any violation of the program semantics.

==> Charts/Behavior_Preserving_Approach_Tree_Structure.tex <==
\dirtree{%
.1 Behavior-Preserving Transformation Approaches.
.2 Refactoring Formalisms and Techniques.
.3 Graph Transformation.
.3 Type Constraints.
.3 Formal Specification and Verification.
.3 Model Transformation.
.4 Model Refactoring and Model Refinement.
.4 Model Driven Refactoring.
.3 Differential Precondition Checking.
.3 Decomposition and Schemes.
.3 Overly Strong Conditions Identification.
.3 Precondition Examination.
.2 Automated Analyses.
.3 Refactoring Safety Tools.
.4 SafeRefactor.
.4 SafeRefactorImpact.
.3 Commit Message Analysis.
.2 Manual Analysis.
}


==> Sections/RunningExample.tex <==
\section{Running Example}
\label{sec:Running Example}
In this section, we demonstrate an example that will be used throughout the paper. The example in Listing~\ref{beforerefactoring} and~\ref{afterrefactoring} illustrates unexpected behavioral changes performed by Eclipse. The original and resulting program are shown with a diff view in which green is for inserts and red is for deletions. 

Consider class \texttt{Employee} and its subclass \texttt{Salesman} as illustrated in Listing~\ref{beforerefactoring}. 
%Class \texttt{Employee} declares the \texttt{getName}, \texttt{getSalary}, \texttt{yearlySalary} methods, and 
 Class \texttt{Salesman} declares methods \texttt{setSSN}, \texttt{getSSN}, \texttt{getFullName}, \texttt{getSalary}, \texttt{getSomething}, \texttt{toString}, \texttt{yearlySalary}, \texttt{yearlySalaryIncrease}, \texttt{displayYearlySalaryIncrease}, \texttt{test1}, and \texttt{test2}. Running the method \texttt{getSomething} in Listing~\ref{beforerefactoring} yields 1000.33. Suppose we want to apply the \textit{PullUpMethod} refactoring using Eclipse to move method \texttt{getSomething} from \texttt{Salesman} to \texttt{Employee}. This method contains a reference to \texttt{Employee.getSalary} using the \texttt{super} access. The use of Eclipse will produce the program presented in Listing~\ref{afterrefactoring}. Although method \texttt{getSomething} is moved to the superclass and \texttt{super} is updated to \texttt{this},  a behavioral change was introduced (i.e., method \texttt{test1} in the target program (Listing~\ref{afterrefactoring}) yields 2000.90 instead of 1000.33). %\Christian{I don't understand this example. I think rewriting it to lean more heavily on Listing 2 would be better. Instead of writing out "Class employee declares getname, getsalary" etc etc, just point the reader at Listing 2 and tell them what they should pay attention to. In particular, it looks like you mostly want them to stare at 'getSomething' and how it is changed from the original code. I'm also a bit confused as to why this pullup method changed the value (without looking at the code). Should mention that, too; make the reader do as little work as possible. \eman{done}}

In this paper, we present how each of the approaches can help to guarantee behavior preservation. %\Christian{is it possible to highlight what between the two listings? \eman{Done}}

\begin{figure*}[htbp]
\noindent\begin{minipage}[t]{.48\textwidth}
%%begin novalidate
\begin{lstlisting}[caption={Original Program},label=beforerefactoring, frame=single,language=diff]{Name}@@ -85,8 +85,8 @@
public class Employee {
	public double yearlySalary;
	public String getName() 
	{	return "John";}
    public double getSalary() 
    {	return 1000.33;}
    public double yearlySalary() {
        return yearlySalary= 
        (getSalary() * 12);
    }
}
 



public class Salesman extends Employee 
	{public String ssn;
	public void setSSN(String setSNN) 
	{	ssn=setSNN;}
	public String getSSN() 
	{	return ssn;}
	public String getFullName() 
	{	return "John Smith";}
	public double getSalary() 
	{	return 2000.99;	}
+	public double getSomething() {
+		return super.getSalary();
+	}
	public String toString() {
		return "Employee[Salary="
		+getSalary()+"]";
	}
    public double yearlySalary() {
        double yearlySalary;
        yearlySalary=(getSalary()*12);
        return yearlySalary;
    }
    public double yearlySalaryIncrease() 
    {    double yearlySalaryIncrease;
        yearlySalaryIncrease = 
        (((yearlySalary()*
        (0.1)) + yearlySalary()));
        return yearlySalaryIncrease;
    }
    public void 
    displayYearlySalaryIncrease() {
        System.out.printf
        ("Yearly Salary Increase 
        is"+yearlySalaryIncrease());
    }
	public double test1() {
		return getSomething();
	}
	public String test2() {
		return getName();
	}
}
public class TestRefactoring {
    public static void main
    (String[] args) {			
    Salesman s=new Salesman();
    System.out.println(s.toString());
+   System.out.println(s.test1());	
    System.out.println(s.test2());	 
	}
}
\end{lstlisting}
%%end novalidate
\end{minipage}%
\hfill
%\hfill\vrule\hfill
%
\begin{minipage}[t]{.48\textwidth}
%%begin novalidate
\begin{lstlisting}[caption={Resulting Program},label=afterrefactoring,frame=single, language=diff]{Name}@@ -85,8 +85,8 @@
public class Employee {
	public double yearlySalary;
	public String getName() 
	{	return "John";}
    public double getSalary() 
    {	return 1000.33;}
    public double yearlySalary() {
        return yearlySalary= 
        (getSalary() * 12);
    }
+   public double getSomething() {
+		return this.getSalary();
+	}
}

public class Salesman extends Employee 
	{public String ssn;
	public void setSSN(String setSNN) 
	{	ssn=setSNN;}
	public String getSSN() 
	{	return ssn;}
	public String getFullName() 
	{	return "John Smith";	}
	public double getSalary()
	{	return 2000.99;}
-	public double getSomething() {
-	    return super.getSalary();
-	}
	public String toString() {
		return "Employee[Salary="
		+getSalary()+"]";
	}
    public double yearlySalary() {
        double yearlySalary;
        yearlySalary=(getSalary()*12);
        return yearlySalary;
    }
    public double yearlySalaryIncrease() 
    {    double yearlySalaryIncrease;
        yearlySalaryIncrease = 
        (((yearlySalary()* 
        (0.1)) + yearlySalary()));
        return yearlySalaryIncrease;
    }
    public void 
    displayYearlySalaryIncrease() {
        System.out.printf
        ("Yearly Salary Increase
        is"+yearlySalaryIncrease());
    }
	public double test1() {
		return getSomething();
	}
	public String test2() {
		return getName();
	}
}
public class TestRefactoring {
    public static void main
    (String[] args) {			
    Salesman s=new Salesman();
    System.out.println(s.toString());
+   System.out.println(s.test1());	
    System.out.println(s.test2());	 
	}
}
\end{lstlisting}
%%end novalidate
\end{minipage}%

\end{figure*}


==> Sections/draft.tex <==
\section{Discussion}
\label{sec:AnalysisDiscussion}
%\eman{if you have idea about additional open issues, please add it in this section}
%This section discusses the results reported in Section~\ref{sec:Results}. A summary of the findings is reported in Table~\ref{Table:Summary}.

\subsection{Software Artifacts (Related to RQ1)}
As reported in Section~\ref{Result:RQ1}, only two software artifacts were considered in the PSs (i.e., code and model). Support for source code and model refactoring have been provided with several language paradigms and programming and modeling languages. Most (83\%) of the PSs were about refactored source code, and a few (17\%) concerning refactored design models. Articles optimizing code are primarily focused on Java programming language. Few articles, however, used C++, Smalltalk, AspectJ, Fortran, PHP, BC, and Erlang to test behavior preservation. For model refactoring, research deals with Alloy specification language or UML models. The focus on Java language might be because of the popularity of Java, and refactoring examples in Fowler's book are written in Java. Researchers are encouraged to focus on different languages and apply more refactoring to design models when testing behavior preservation. 

\subsection{Refactoring Activities (Related to RQ2)}
The PSs addressed 101 refactoring operations when testing the behavior preservation of the program. We classify these refactorings into three categories: refactorings proposed by Fowler, refactorings applied in design model, and refactorings related to specific programming languages. We found that refactorings fall into the first category were used more frequently (i.e., 52\% of the PSs). 41\% of PSs used refactoring operations related to specific languages. The remaining model refactorings were studied far less frequently (7\% of the PSs).

The results in Figure~\ref{Chart:RefactoringsOccurrence} partially match the findings in previous research (e.g., \cite{6112738}\cite{bavota2012does}) in terms of the most popular refactoring types used in the literature. It is worth noting that some refactorings from Fowler's catalog were used far more frequently than refactorings from other categories. The high interest in these refactoring operations may indicate their importance in preserving the behavior and are potentially more frequently applied in practice than other refactoring operations. %The full list of refactorings considered by each PS is available on Google Docs.


\subsection{Behavior Preservation Approaches (Related to RQ3)}

Today, a wide variety of refactoring tools automates several aspects of refactoring. However, ensuring the behavior preserving property when building tool-assisted refactoring is challenging. It is acknowledged that refactoring tools should support the following five characteristics: automation, reliability, configurability, coverage, and scalability. Integrating behavior-preserving nature reduces the need to perform testing and debugging. 


Several formalisms and techniques have been proposed in the existing literature to guarantee the behavior preservation and correctness of refactorings. Actual source code transformation and a set of preconditions are the two main parts for any refactoring operation to be performed by automated refactorings. 

As shown in Table~\ref{Table:Behavior_Preservation_Approaches_Subcategories.}, the most frequently used approaches are precondition-based and testing-based. All of the remaining approaches have almost similar frequency. Several precondition-oriented approaches were defined in the literature. Overbey and Johnson \cite{6100067} propose a practical technique to enable checking many compilability and preservation preconditions after the transformation. This technique represents the program as a graph and is language-independent which is a crucial characteristic for any tool support or formal model for refactoring.  Garrido and Meseguer \cite{4026866} introduce rewrite logic semantics to formally specify Java refactorings and to reach a precise specification of the preconditions. This formal technique needs to be improved to make the technology more generic, and the library needs to be extended to include more refactorings. Due to the limitation of the current specification in refactoring tools (e.g., language specific and inaccurate specification), Mens et al. suggest using a formal model defining the effects of refactoring activity in the source code. This formalism incorporates the use of both graph rewriting rules and assertions (i.e. preconditions and postconditions) as a formal specification for refactoring. This formal model can improve reliability, which is another important characteristic to guarantee that its refactoring behaviorally preserves transformations. Further, in \cite{4752842}, a set of behavior preservation precondition examinations were proposed for \textit{Move Method} refactoring. This approach helps in eliminating the \textit{feature envy} bad smell and leads to a positive impact on both the cohesion and coupling internal quality attributes. To verify preconditions of refactorings, Tip et al. \cite{Tip:2003:RGU:949305.949308} proposed the use of type constraints that depend on interprocedural relationships between variable types. 

Moreover, contemporary IDEs such as Eclipse and IntelliJ that support refactoring often allow erroneous transformations to be applied which cause a behavior change. To avoid behavioral changes in these automated refactorings, safety refactoring tools are introduced in \cite{article} \cite{Mongiovi:2014:MRS:2664678.2664813} . This practice relies on generating unit tests for checking refactoring safety and detecting behavioral changes during program transformations. Beside ensuring behavior preservation in refactoring implementations,  a set of preconditions needs to be checked to ensure useful transformation to be behavior-preserving based on differential testing and disabling precondition. Developers can use these approaches as a complement to the traditional refactoring steps to have extra confidence about the correctness and preservation of the transformations; in addition, to formally specify conditions that may lead to non-behavior preserving transformations to be performed. To ensure the accuracy of the transformation, Horpácsi et al. \cite{Horpcsi2017TrustworthyRV} propose decomposing complex refactoring into several micro refactorings that can be easily verified. Furthermore, commit message analysis is another automated approach to identify behavior-preserving transformations in software repositories. Although this approach is simple and fast, when conducting experiment in \cite{SOARES20131006}, it is  found that this approach fails to predict a number of behaviorally preserving transformations. Additionally, Murphy-Hill et al. \cite{6112738} found that commit messages are unreliable indicators of refactorings because developers tend to not state refactoring activity when committing new changes. In contrast to the automated analyses, the manual analysis approach is reliable and easily understandable since it decomposes the transformation into minor changes \cite{6112738}. The drawback with the manual approach, however, is that it is time consuming, can be error-prone, and highly depends on evaluators' experience when analyzing the source code.   

With respect to model refactoring, Massoni et al. \cite{Massoni:2008:FMP:1792838.1792873} suggest a formal approach to refactor programs in a model-driven manner. Instead of generating changes to a program from models which involve manual updates, this formalism suggests refactoring only object models and keeps these object models in conformance to their implementations by semi-automatic refactoring, avoiding the need to update source code manually. Further, Straeten et al. \cite{VanDerStraeten2007} explore the relations between the notion of behavior inheritance consistency of model refinement and behavior preservation of model refactoring, and found that strong correlation exists between these two notions. 

%In some related areas, such as software refactoring and quality measurement, the obtained data and results are available in online repositories to facilitate reproducability and replicability of the results. We are not aware of similar repositories in the area of behavior preservation in software refactoring. Researchers are advised to make the obtained data of the proposed behavior preserving techniques available online in public repositories so that other researchers can use these data as benchmarks for comparison with their obtained results. %Since these tools are not available, it hinders their applicability and does not help any IDE to adopt that.



\subsection{Evaluation Methods (Related to RQ4)}
The results reported in Section~\ref{Result:RQ4} show that 15 of the PSs applied a variety of evaluation methods to assess the proposed behavior preservation approaches including comparison-based, empirical-based, formal specification-based, quality-based, and independent-assessment based evaluation methods. Also, a future validation tool was suggested in one of the PSs (\cite{Mens2003FormalisingRW}) to evaluate the approach. The most used method is the empirical-based followed by the comparison-based and formal-specification-based evaluation. One of the PSs (\cite{4752842}) applied two evaluation methods, and all of the remaining PSs considered only one method. Researchers are encouraged to apply one or more of these evaluation methods when proposing behavior-preserving transformation techniques.   


%\input{Tables/Summary}








==> Tables/Automated_Tools_Comparison.tex <==
\begin{table}[h]
\begin{center}
\caption{Refactoring Safety Tools Comparison.}
\label{Table:Refactoring_Safety_Tools_Comparison}
\begin{adjustbox}{width=1.0\textwidth,center}
\begin{tabular}{lll}
%{p{3cm}p{2.9cm}p{3cm}}\hline
\toprule
\bfseries Tool & \bfseries SafeRefactor & \bfseries SafeRefactorImpact \\
\midrule
Technology & OOP & OOP \& AOP   \\
Methods Detected & common methods & methods impacted by transformation \\
Test Cases Generated & relevant \& non-relevant test cases & relevant test cases \\ 
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}

==> Tables/Behavior_Preserving_Approach_2.tex <==
\begin{table*}[h]
\begin{center}
\caption{Behavior Preservation Approaches and its Subcategories. \eman{needs to be updated}}
\label{Table:Behavior_Preservation_Approaches_Subcategories.}
\begin{adjustbox}{width=1.0\textwidth,center}
\begin{tabular}{p{4.5cm}  p{4cm} p{3cm} p{6cm} }\hline
\toprule
\multicolumn{1}{l}{\bfseries {Approach}}  & \bfseries Subcategories  & \bfseries No. of PSs & \bfseries  PSs  \\
\midrule
\multirow{4}{*}{Formalisms \& Techniques} & Precondition-based & 7 & \cite{Mens2003FormalisingRW}\cite{Tip:2003:RGU:949305.949308} \cite{4752842}\cite{6100067}\cite{6080784}\cite{7898404}\cite{4026866}  \\ 
& Graph-based & 2 & \cite{Mens2003FormalisingRW} \cite{6100067}\\ 
& Model-based & 2 & \cite{Massoni:2008:FMP:1792838.1792873} \cite{VanDerStraeten2007}  \\ 
& Decomposition-based & 2 &  \cite{Horpcsi2017TrustworthyRV}\cite{Massoni:2008:FMP:1792838.1792873} \\ %\hline
& & &  \\
\multirow{2}{*}{Automated Approach} & Testing-based & 6 & \cite{article} \cite{soares2009generating}\cite{5440166}\cite{SOARES20131006}\cite{Mongiovi:2014:MRS:2664678.2664813}\cite{soares2011making}  \\ 
& Precondition-based & 1 & \cite{roberts1997refactoring} \\
& Keywords-based & 1 & \cite{SOARES20131006}  \\
& & &  \\
\multirow{1}{*}{Manual Approach} & Comparison-based & 1 & \cite{SOARES20131006}  \\ 
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\end{table*}

==> Tables/CommitClassificationExample.tex <==
\begin{table*}[]
  \centering
	 \caption{Commits Message Example.}
	 \label{Table:Commits_Messages_Example}
%\begin{sideways}
\begin{adjustbox}{width=1.1\textwidth,center}
\begin{tabular}{llll}
\toprule
\bfseries Category & \bfseries Subcategory & \bfseries \begin{tabular}[c]{@{}l@{}}Refactoring Operation\end{tabular}                                                                                                                                                           & \bfseries \begin{tabular}[c]{@{}l@{}}Commit Messages\end{tabular}                                                                                                                                                               \\ 
\midrule
Feature  & \begin{tabular}[c]{@{}l@{}}Feature Addition\\    \\    \\   Feature Modification\\    \\    \\    \\   Feature Deletion\end{tabular}                                                                                        & \begin{tabular}[c]{@{}l@{}}Rename \& Extract Method\\    \\    \\   Rename Method\\    \\    \\    \\   Pull Up Attribute\end{tabular}                                                                              & \begin{tabular}[c]{@{}l@{}}\\ Implementation of the feature to allow user to add custome exception. Code refactoring for various modules. Incorporated Fabios’s old\\   review comment. \\    \\   Feature \#5157 - refactoring of album view page (adding some string templates) (modifying homepage) (modifying the view of a photo)\\   (fixing search result display problems)\\    \\   Refactored the sauce test class to a base and subclass with test content. Reused sauce base test class to run session id and job-name printing test and checking output by capturing stdout. \\ The nature of the feature being tested forced some unorthodox testing. Also removed build id update from the SauceOnDemandTestListener class to give user the freedom to set their own.\\ In the earlier setup the Jenkins tag was   overwriting the user set one causing odd behaviour.\\ \end{tabular} \\ \\ \hline

BugFix   & \begin{tabular}[c]{@{}l@{}}Bug Resolution \\    \\   Bug   Resolution \\    \\   Bug Resolution \\    \\       Debugging\\    \\   Bug Localization\end{tabular}                                                    & \begin{tabular}[c]{@{}l@{}}Extract Method\\    \\   Rename Method\\    \\   Extract Method \\    \\       Move \& Rename Class\\    \\   Move Method\end{tabular}                                       & \begin{tabular}[c]{@{}l@{}}\\ Refactoring of SlidingWindow class in RR to reduce complexity and  fix important bug, \\    \\   Fixed a bug in Extract Function refactoring.\\    \\   Refactor the code to fix bug 256238,Shouldn't update figure before inserting extended item such as Chart in library editor\\    \\   Renaming and refactoring towards debugging  functionality\\    \\   Moved generateObjects() from AbstractFunction to FunctionHelper. More natural. Updated Wiki docs to reflect this. Found a bug   with using variables in predicates. \\ commented out the test case that breaks. Added some test cases that are more complicated uses of ScriptEngine.
\end{tabular}                                               \\ \\ \hline
Design   & \begin{tabular}[c]{@{}l@{}}\\ Remove Long Method\\    \\   Remove Duplication\\    \\   Remove Data Class\\    \\   Inheritance \\    \\       Code Smell Resolution \\    \\   Remove Feature Envy\end{tabular} & \begin{tabular}[c]{@{}l@{}}\\ Extract Method\\    \\   Extract Method\\    \\   Move Class\\    \\   Move Attribute, Rename \& Move Method\\    \\   Extract  Method \\    \\   Move Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}\\ MongoStore: Refactor to avoid long methods\\    \\   Minor refactoring to remove duplicate code\\    \\   Refactoring of core data classes. Implementation of RefactoringRegistry.\\    \\   Refactoring of filters to make better use of  inheritance hierarchy.\\    \\       Fix code smells. \\    \\   Introduced adjuncts from stapler - fixed the feature envy problem in the version computation
\end{tabular}  
\\ \\  \hline

Non-Functional & \begin{tabular}[c]{@{}l@{}}\\ Testability\\    \\   Usability\\    \\   Performance\\    \\   Reusability \\    \\   Readability\end{tabular}                                                                                          & \begin{tabular}[c]{@{}l@{}}\\ Extract Method \\    \\   Rename Method\\    \\   Extract   Method \\    \\   Move Method \\    \\   Extract Method\end{tabular}                                                       & \begin{tabular}[c]{@{}l@{}}\\ Minor refactoring for better testability without the need to generate intermediary files.\\    \\   Refactor: Remove redundant method names, improve usability. \\   \\     Improve performance of MessageSource condition.\\   \\   Refactored for better reusability.\\    \\   Refactoring mostly for readability (and small performance improvement)\end{tabular}   \\ \\               
\bottomrule
\end{tabular}
\end{adjustbox}
%\end{sideways}
\end{table*}

==> Tables/Quality_Assessment_Answer.tex <==
\begin{table*}[h]
\begin{center}
\caption{PS Quality Assessment Answers. }
\label{Table:Quality_Assessment_Answers}
%\begin{adjustbox}{width=1.0\textwidth,center}
\begin{adjustbox}{width=0.9\textwidth,center}
\begin{tabular}{llllllllllllll}\hline
\toprule
\bfseries Study & \bfseries QA1 & \bfseries QA2 & \bfseries QA3 & \bfseries QA4 & \bfseries QA5 & \bfseries QA6 & \bfseries QA7 & \bfseries QA8 & \bfseries QA9 & \bfseries QA10 & \bfseries QA11 & \bfseries QA12 & \bfseries QA13 \\
%\multicolumn{2}{r}{\textbf{\textit{Q1}}}\\
\midrule
Roberts et al. \cite{roberts1997refactoring} & 1 & 1 & 0.5 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 0 & 0 \\
Mens et al. \cite{Mens2003FormalisingRW} & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 0 & 1 \\
Tip et al. \cite{Tip:2003:RGU:949305.949308} & 1 & 1 & 0.5 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 0 & 0 & 0    \\
%Mens and Tourwe \cite{1265817} & 1 & 1 & 0.5 & 1 & 1 & 1 & 1 & 0 & 0 & 1 & 0.5 & 1 & 0.5  \\
Garrido and Meseguer \cite{4026866} & 1 & 1 & 0.5 & 1  & 0 & 1 & 0.5 & 0 & 0 & 1 & 0 & 0 & 0  \\
Straeten et al. \cite{VanDerStraeten2007} & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 0 & 1  \\
Massoni et al. \cite{Massoni:2008:FMP:1792838.1792873} & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 0 & 0 \\
Soares et al. \cite{article} & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 0 & 0 & 0   \\
Soares et al. \cite{soares2009generating} & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 0 & 0 & 0 \\
Tsantalis and Chatzigeorgiou \cite{4752842} & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 0 & 1 \\
Soares et al. \cite{5440166} & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 0 & 1 & 0  \\
Soares et al. \cite{soares2011making} & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 0 & 1  \\ 
Overbey and Johnson \cite{6100067} & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 0 & 1   \\
Soares et al. \cite{6080784} & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 0 & 0 & 0\\
Soares et al. \cite{SOARES20131006} & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 1 & 1 \\
Mongiovi et al. \cite{Mongiovi:2014:MRS:2664678.2664813} & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 0 & 1 & 1 \\
Horpácsi et al. \cite{Horpcsi2017TrustworthyRV} & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 0 & 0 & 0 \\ 
Mongiovi et al. \cite{7898404} & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 0.5 & 1 & 1 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\end{table*}

==> Tables/Quality_Assessment_Question.tex <==
\begin{table*}[h]
\begin{center}
\caption{PS Quality Assessment Questions. }
\label{Table:Quality_Assessment_Questions}
\begin{adjustbox}{width=0.9\textwidth,center}
\begin{tabular}{ll}\hline
\toprule
\bfseries ID & \bfseries Question \\
\midrule
\multicolumn{2}{l}{\textbf{\textit{Design}}}\\
QA1 & Are the aims clearly stated?\\
QA2 & Was the study designed with these questions in mind?\\
QA3 & Are the considered approaches/measures in the study fully defined? \\
QA4 & Do the study measures allow questions to be answered? \\
\midrule 
\multicolumn{2}{l}{\textbf{\textit{Conduct}}}\\
QA5 & Are the data collection methods adequately described?  \\
\midrule
\multicolumn{2}{l}{\textbf{\textit{Analysis}}}\\
QA6 & Is the purpose of the analysis clear? \\
QA7 & Were the basic data adequately described? \\
QA8 & Are the statistical methods described? \\
QA9 & Are the statistical methods justified? \\
\midrule
\multicolumn{2}{l}{\textbf{\textit{Conclusion}}}\\
QA10 & Are all study questions answered? \\
QA11 & Are negative finding presented? \\
QA12 & Are the results compared with previous reports?\\
QA13 & Do the researchers explain the consequences of any problems with the validity/reliability of their measures?\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\end{table*}

==> Tables/Refactoring_Operation.tex <==
\begin{center}
\clearpage
\onecolumn
\begin{longtable}{l|l|l}
\caption{Refactoring Operations in Related Work.} \label{Table:Refactoring_Operation} \\

\hline \multicolumn{1}{c|}{\textbf{Study}} & \multicolumn{1}{c|}{\textbf{Approach}} & \multicolumn{1}{c}{\textbf{Refactorings}}\\ \hline 
\endfirsthead

\multicolumn{3}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline \multicolumn{1}{c|}{\textbf{Study}} & \multicolumn{1}{c|}{\textbf{Approach}} & \multicolumn{1}{c}{\textbf{Refactorings}} \\ \hline 
\endhead

\hline \multicolumn{3}{|r|}{{Continued on next page}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

Mens et al. \cite{Mens2003FormalisingRW} & Graph Transformation & Encapsulate Field \\ 
& & Pull Up Method  \\ \hline
Tip et al. \cite{Tip:2003:RGU:949305.949308} & Type Constraints  & Generalization-related Refactorings  \\ \hline
Garrido and Meseguer \cite{4026866} & Formal Specification \& Verification & Push Down Method  \\ 
& & Pull Up Field  \\ 
& & Rename Temporary  \\\hline
Straeten et al. \cite{VanDerStraeten2007} &  Model Transformation & Move States into Orthogonal Composite State   \\ 
& & Flatten States  \\
& & Add Subclass  \\\hline
Massoni et al. \cite{Massoni:2008:FMP:1792838.1792873} & Model Transformation  & Introduce Signature  \\ 
             & & Introduce Generalization  \\
             & & Introduce Subsignature  \\
             & & Introduce Relation  \\
             & & Remove Optional Relation  \\ 
             & & Remove Scalar Relation  \\ 
             & & Split Relation  \\ \hline
Soares et al. \cite{article} & Safe Refactoring Tools & Push Down Method  \\
Soares et al. \cite{soares2009generating} & & Rename Class  \\
Soares et al. \cite{5440166} & & Rename Field  \\
 & & Rename Local Variable  \\
 & & Rename Method  \\
 & & Encapsulate Field  \\
 & & Extract Method  \\ 
 & & Extract Class \\ 
 & & Move Class  \\
 & & Change Method Signature  \\
 & & Pull Up Method \\ 
 & & Extract Exception Handler \\
& & Infer Generic Type \\
& & Replace Deprecated Code \\ \hline             
Tsantalis and Chatzigeorgiou \cite{4752842} & Precondition Examination & Move Method \\ \hline
Overbey and Johnson \cite{6100067} &  Differential Precondition Checking & Rename     \\ 
& & Move  \\
& & Introduce USE  \\
& & Change Function Signature  \\
& & Introduce Implicit None  \\
& & Add Empty Subprogram  \\
& & Safe Delete  \\
& & Pull Up Method  \\
& & Copy Up Method  \\
& & Extract Local Variable  \\ 
& & Add Local Variable  \\
& & Introduce Block  \\
& & Insert Assignment  \\
& & Move Expression   \\
& & Extract Function  \\ 
& & Add Empty Function  \\ 
& & Populate Function  \\
& & Replace Expression  \\
\hline
Soares et al. \cite{6080784} & Overly Strong Conditions Identification & Pull Up Field  \\ 
Mongiovi et al. \cite{7898404} & & Pull Up Method \\ 
& & Rename Method \\ 
& & Move Method \\
& & Push Down Field \\ 
& & Push Down Method \\ 
& & Add Parameter \\ 
& & Encapsulate Field \\ 
& & Rename Field \\ 
& & Rename Type \\ \hline
Soares et al. \cite{SOARES20131006} & Manual Analysis & Replace Code with Method Call \\
& & Move Operation to Listener  \\
& & Extract Method  \\
& & Remove Unused Variable  \\
& & Change Instance Access to Static  \\
& & Remove Immutable Object Copy  \\
& & Replace Direct Access with Getter  \\
& & Replace Instance with isInstance  \\
& & Add Parameter  \\
& & Remove Parameter  \\
& & Replace Field with Method  \\
& & Decrease Method Visibility  \\
& & Replace Direct Access with Setter  \\
& & Inline Temp \\
& & Move Method \\
& & Consolidate Duplicate Code Fragment \\
& & Rename Constant \\
& & Rename Local Variable \\
& & Replace Generic Cast with classCast  \\
& & Replace Generic Cast with isInstance \\
& & Replace Method with Method Object \\
& & Change Statement Order \\
& & Swap Access Method \\
& & Remove Duplicate Assignment \\
& & Consolidate Conditional Expression \\
& & Introduce Explaining Variable \\
& & Remove Assignment to Parameters \\
& & Rename Class\\
& & Increase Method Visibility \\
& & Rename Method \\
& & Rename Field \\
& & Replace if with Switch \\
& & Replace Equivalent Method Call \\
& & Introduce Null Object \\
& & Replace Magic Number with Constant \\
\hline
Mongiovi et al. \cite{Mongiovi:2014:MRS:2664678.2664813} & Safe Refactoring Tool & Add Method \\
& & Remove Method \\
& & Change Method Body \\
& & Change Method Modifier \\
& & Add Field \\
& & Remove Field \\
& & Change Field Modifier \\
& & Change Field Initializer \\
& & Change Static Field Initializer \\
& & Rename Class \\
& & Rename Method \\
& & Rename Field \\
& & Rename Intertype Declaration \\
& & Push Down Method \\
& & Pull Up Method \\
& & Inline Method \\
Horpácsi et al. \cite{Horpcsi2017TrustworthyRV} &  Decomposition \& Schemes & Wrap (Change) Expression \\ 
                & & Extract to Function \\ 
                & & Extract to Variable \\
                & & Outer Variable \\
                & & Variable to Function Parameter \\
                & & Rename Function \\
\end{longtable}
\clearpage
\twocolumn
\end{center}

==> Tables/ResearchQuestion_PICOC.tex <==
\begin{table*}[h]
\begin{center}
\caption{Mapping between the PICOC Criteria \& Research Questions. }
\label{Table:PICOC_Research_Questions}
\begin{adjustbox}{width=1.0\textwidth,center}
\begin{tabular}{l p{12cm} l}\hline
\toprule
\bfseries PICOC Criterion & \bfseries Addressed Research Problems & \bfseries  Research Question \\
\midrule
\multicolumn{2}{l}{\textbf{\textit{Population}}}\\
& Refactoring operations considered by the PSs & RQ2  \\
\midrule 
\multicolumn{2}{l}{\textbf{\textit{Intervention}}}\\
& Approaches and evaluation methods considered by the PSs to assess the behavior-preserving transformations & RQ3 and RQ4  \\
\midrule
\multicolumn{2}{l}{\textbf{\textit{Comparison}}}\\
& N/A & N/A\\
\midrule
\multicolumn{2}{l}{\textbf{\textit{Outcomes}}}\\
& A categorization of the behavior preservation approaches & RQ3 \\ 
\midrule
\multicolumn{2}{l}{\textbf{\textit{Context}}}\\
& Context in terms of the software artifacts and the language paradigm covered by the PSs & RQ1\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\end{table*}
